Optical-Ultraviolet Tidal Disruption Events

The existence of optical-ultraviolet Tidal Disruption Events (TDEs) could be considered surprising because their electromagnetic output was originally predicted to be dominated by X-ray emission from an accretion disk. Yet over the last decade, the growth of optical transient surveys has led to the identification of a new class of optical transients occurring exclusively in galaxy centers, many of which are considered to be TDEs. Here we review the observed properties of these events, identified based on a shared set of both photometric and spectroscopic properties. We present a homogeneous analysis of 33 sources that we classify as robust TDEs, and which we divide into classes. The criteria used here to classify TDEs will possibly get updated as new samples are collected and potential additional diversity of TDEs is revealed. We also summarize current measurements of the optical-ultraviolet TDE rate, as well as the mass function and luminosity function. Many open questions exist regarding the current sample of events. We anticipate that the search for answers will unlock new insights in a variety of fields, from accretion physics to galaxy evolution.

==> Overleaf arXiv Submission Generated source/tables/info_ISSI.tex <==
SDSS-TDE2            &                 & 23:23:48.61\,$-$01:08:10.2  & 2007-06-15$^*$ &   0.2515  & $-21.3$ & H                                  &  $10.57_{0.10}^{0.17}$ & 1\\
PTF-09ge             &                 & 14:57:03.18\,$+$49:36:40.9  & 2009-06-10~    &    0.064  & $-19.8$ & He~(Fe?)                           &  $10.11_{0.12}^{0.13}$ & 2\\
PTF-09axc            &                 & 14:53:13.07\,$+$22:14:32.2  & 2009-07-04~    &   0.1146  & $-19.5$ & H                                  &  $10.12_{0.17}^{0.11}$ & 2\\
PTF-09djl            &                 & 16:33:55.97\,$+$30:14:16.6  & 2009-08-05~    &    0.184  & $-20.3$ & H                                  &  $9.95_{0.12}^{0.15}$ & 2\\
PS1-10jh             &                 & 16:09:28.27\,$+$53:40:23.9  & 2010-07-16~    &   0.1696  & $-19.6$ & He                                 &  $9.61_{0.13}^{0.10}$ & 3\\
PS1-11af             &                 & 09:57:26.81\,$+$03:14:00.9  & 2011-01-17~    &   0.4046  & $-20.2$ & Unknown                            &  $10.21_{0.19}^{0.21}$ & 4\\
ASASSN-14ae          &                 & 11:08:40.11\,$+$34:05:52.2  & 2014-01-27$^*$ &   0.0436  & $-19.6$ & H\,$\rightarrow$\,H+He             &  $10.02_{0.17}^{0.09}$ & 5\\
ASASSN-14li          &                 & 12:48:15.23\,$+$17:46:26.4  & 2014-11-28$^*$ &  0.02058  & $-18.1$ & H+He~(N)                           &  $9.69_{0.10}^{0.05}$ & 6\\
iPTF-15af            &                 & 08:48:28.13\,$+$22:03:33.4  & 2015-02-08~    &  0.07897  & $-18.0$ & H+He~(N+O)                         &  $10.33_{0.18}^{0.11}$ & 7\\
ASASSN-15oi          &                 & 20:39:09.14\,$-$30:45:20.6  & 2015-08-13$^*$ &   0.0484  & $-21.9$ & He~(Fe?+O?)                           &  $10.02_{0.04}^{0.04}$ & 8\\
OGLE16aaa            &                 & 01:07:20.76\,$-$64:16:20.4  & 2016-01-27~    &   0.1655  & $-20.7$ & H+He                              &  $10.47_{0.11}^{0.09}$ & 9\\
iPTF-16axa           &                 & 17:03:34.34\,$+$30:35:36.6  & 2016-05-15$^*$ &    0.108  & $-19.0$ & H+He~(N+O?)                           &  $10.18_{0.14}^{0.10}$ & 10\\
iPTF-16fnl           &                 & 00:29:57.05\,$+$32:53:37.2  & 2016-08-26~    &   0.0163  & $-17.5$ & H+He~(N)                           &  $9.35_{0.15}^{0.12}$ & 11\\
PS17dhz              & AT\,2017eqx     & 22:26:48.37\,$+$17:08:52.3  & 2017-06-06~    &   0.1089  & $-18.8$ & H+He\,$\rightarrow$\,He~(N+Fe?)    &  $9.44_{0.13}^{0.11}$ & 12\\
PS18kh               & AT\,2018zr      & 07:56:54.54\,$+$34:15:43.6  & 2018-03-03~    &    0.071  & $-19.9$ & H                                  &  $10.03_{0.18}^{0.09}$ & 13\\
ZTF18aahqkbt         & AT\,2018bsi     & 08:15:26.63\,$+$45:35:32.0  & 2018-04-09$^*$ &    0.051  & $-19.0$ & H+He~(N)                           &  $10.61_{0.06}^{0.05}$ & 14\\
ASASSN-18ul          & AT\,2018fyk     & 22:50:16.09\,$-$44:51:53.5  & 2018-07-18$^*$ &    0.059  & $-19.6$ & H+He~(O+Fe)                        &  $10.57_{0.21}^{0.12}$ & 15\\
ASASSN-18pg          & AT\,2018dyb     & 16:10:58.87\,$-$60:55:24.3  & 2018-08-16~    &    0.018  & $-19.8$ & H+He~(N+O)                         &  $9.83_{0.15}^{0.08}$ & 16\\
ATLAS18way           & AT\,2018hco     & 01:07:33.63\,$+$23:28:34.2  & 2018-10-10~    &    0.088  & $-19.4$ & H                                  &  $9.90_{0.18}^{0.09}$ & 14\\
ASASSN-18zj          & AT\,2018hyz     & 10:06:50.88\,$+$01:41:33.9  & 2018-11-05$^*$ &  0.04573  & $-20.3$ & H                                  &  $9.75_{0.26}^{0.12}$ & 14\\
ATLAS18yzs           & AT\,2018iih     & 17:28:03.92\,$+$30:41:31.5  & 2018-11-20~    &    0.212  & $-21.6$ & He                                 &  $10.76_{0.15}^{0.09}$ & 14\\
ZTF18actaqdw         & AT\,2018lni     & 04:09:37.65\,$+$73:53:41.6  & 2018-12-08~    &    0.138  & $-19.4$ & H+He~(N+O)                         &  $9.94_{0.15}^{0.10}$ & 14\\
ZTF19aabbnzo         & AT\,2018lna     & 07:03:18.64\,$+$23:01:44.6  & 2019-01-25~    &    0.091  & $-19.5$ & H+He~(N?)                               &  $9.47_{0.09}^{0.12}$ & 14\\
ZTF19aakswrb         & AT\,2019bhf     & 15:09:15.97\,$+$16:14:22.5  & 2019-02-25~    &   0.1206  & $-20.1$ & H                                  &  $10.21_{0.12}^{0.15}$ & 14\\
ASASSN-19bt          & AT\,2019ahk     & 07:00:11.39\,$-$66:02:24.7  & 2019-03-06~    &   0.0262  & $-20.7$ & H                                  &  $9.74_{0.10}^{0.09}$ & 17\\
ZTF19aakiwze         & AT\,2019cho     & 12:55:09.20\,$+$49:31:09.9  & 2019-02-21~    &    0.193  & $-20.7$ & H+He~(N)                           &  $10.10_{0.16}^{0.17}$ & 14\\
ASASSN-19dj          & AT\,2019azh     & 08:13:16.95\,$+$22:38:53.8  & 2019-03-16~    &   0.0222  & $-19.9$ & H+He                               &  $9.86_{0.14}^{0.15}$ & 18\\
ZTF19aapreis         & AT\,2019dsg     & 20:57:02.97\,$+$14:12:16.2  & 2019-04-27~    &   0.0512  & $-19.2$ & H+He~(N+O)                         &  $10.36_{0.12}^{0.17}$ & 14\\
Gaia19bpt            & AT\,2019ehz     & 14:09:41.90\,$+$55:29:27.7  & 2019-05-08~    &    0.074  & $-19.6$ & H                                  &  $9.67_{0.15}^{0.09}$ & 14\\
ZTF19abidbya         & AT\,2019lwu     & 23:11:12.30\,$-$01:00:10.8  & 2019-07-26~    &    0.117  & $-19.8$ & H                                  &  $9.87_{0.15}^{0.12}$ & 14\\
ZTF19abhhjcc         & AT\,2019meg     & 18:45:16.19\,$+$44:26:18.9  & 2019-08-01~    &    0.152  & $-20.2$ & H                                  &  $9.69_{0.05}^{0.05}$ & 14\\
ATLAS19qqu           & AT\,2019mha     & 16:16:27.78\,$+$56:25:56.3  & 2019-08-09~    &    0.148  & $-19.9$ & H                                  &  $10.05_{0.15}^{0.11}$ & 14\\
ZTF19abzrhgq         & AT\,2019qiz     & 04:46:37.88\,$-$10:13:34.8  & 2019-10-05~    &   0.0151  & $-18.6$ & H+He~(N)                           &  $10.03_{0.14}^{0.10}$ & 14\\
% SDSS-TDE2            &                 & 23:23:48.61\,$-$01:08:10.2  & 2007-06-15  &   0.2515  & $-21.3$ & H                 &  $10.57_{0.10}^{0.17}$ & 1\\
% PTF-09ge             &                 & 14:57:03.18\,$+$49:36:40.9  & 2009-06-10  &    0.064  & $-19.8$ & He\,(Fe?)                &  $10.11_{0.12}^{0.13}$ & 2\\
% PTF-09axc            &                 & 14:53:13.07\,$+$22:14:32.2  & 2009-07-04  &   0.1146  & $-19.5$ & H                 &  $10.12_{0.17}^{0.11}$ & 2\\
% PTF-09djl            &                 & 16:33:55.97\,$+$30:14:16.6  & 2009-08-05  &    0.184  & $-20.3$ & H                 &  $9.95_{0.12}^{0.15}$ & 2\\
% PS1-10jh             &                 & 16:09:28.27\,$+$53:40:23.9  & 2010-07-16  &   0.1696  & $-19.6$ & He                &  $9.61_{0.13}^{0.10}$ & 3\\
% PS1-11af             &                 & 09:57:26.81\,$+$03:14:00.9  & 2011-01-17  &   0.4046  & $-20.2$ & Unknown               &  $10.21_{0.19}^{0.21}$ & 4\\
% ASASSN-14ae          &                 & 11:08:40.11\,$+$34:05:52.2  & 2014-01-27  &   0.0436  & $-19.6$ & H\,$\rightarrow$\,H+He                 &  $10.02_{0.17}^{0.09}$ & 5\\
% ASASSN-14li          &                 & 12:48:15.23\,$+$17:46:26.4  & 2014-11-28  &  0.02058  & $-18.1$ & H+He\,(Bowen)     &  $9.69_{0.10}^{0.05}$ & 6\\
% iPTF-15af            &                 & 08:48:28.13\,$+$22:03:33.4  & 2015-02-08  &  0.07897  & $-18.0$ & H+He\,(Bowen)     &  $10.33_{0.18}^{0.11}$ & 7\\
% ASASSN-15oi          &                 & 20:39:09.14\,$-$30:45:20.6  & 2015-08-13  &   0.0484  & $-21.9$ & He\,(Fe?)                &  $10.02_{0.04}^{0.04}$ & 8\\
% OGLE16aaa            &                 & 01:07:20.76\,$-$64:16:20.4  & 2016-01-27  &   0.1655  & $-20.7$ & H+He?             &  $10.47_{0.11}^{0.09}$ & 9\\
% iPTF-16axa           &                 & 17:03:34.34\,$+$30:35:36.6  & 2016-05-15  &    0.108  & $-19.0$ & H+He\,(Bowen)     &  $10.18_{0.14}^{0.10}$ & 10\\
% iPTF-16fnl           &                 & 00:29:57.05\,$+$32:53:37.2  & 2016-08-26  &   0.0163  & $-17.5$ & H+He\,(Bowen)     &  $9.35_{0.15}^{0.12}$ & 11\\
% PS17dhz              & AT\,2017eqx       & 22:26:48.37\,$+$17:08:52.3  & 2017-06-06  &   0.1089  & $-18.8$ & H+He\,$\rightarrow$He\,(Bowen)     &  $9.44_{0.13}^{0.11}$ & 12\\
%  PS18kh              & AT\,2018zr        & 07:56:54.54\,$+$34:15:43.6  & 2018-03-03  &    0.071  & $-19.9$ & H                 &  $10.03_{0.18}^{0.09}$ & 13\\
% ZTF18aahqkbt         & AT\,2018bsi       & 08:15:26.63\,$+$45:35:32.0  & 2018-04-09  &    0.051  & $-19.0$ & H+He\,(Bowen)     &  $10.61_{0.06}^{0.05}$ & 14\\
% ASASSN-18ul          & AT\,2018fyk       & 22:50:16.09\,$-$44:51:53.5  & 2018-07-18  &    0.059  & $-19.6$ & H+He\,(Bowen,\,Fe)     &  $10.57_{0.21}^{0.12}$ & 15\\
% ASASSN-18pg          & AT\,2018dyb       & 16:10:58.87\,$-$60:55:24.3  & 2018-08-16  &    0.018  & $-19.8$ & H+He\,(Bowen)     &  $9.83_{0.15}^{0.08}$ & 16\\
%  ATLAS18way          & AT\,2018hco       & 01:07:33.63\,$+$23:28:34.2  & 2018-10-10  &    0.088  & $-19.4$ & H                 &  $9.90_{0.18}^{0.09}$ & 14\\
%  ASASSN-18zj         & AT\,2018hyz       & 10:06:50.88\,$+$01:41:33.9  & 2018-11-05  &  0.04573  & $-20.3$ & H                 &  $9.75_{0.26}^{0.12}$ & 14\\
%  ATLAS18yzs          & AT\,2018iih       & 17:28:03.92\,$+$30:41:31.5  & 2018-11-20  &    0.212  & $-21.6$ & He                &  $10.76_{0.15}^{0.09}$ & 14\\
% ZTF18actaqdw         & AT\,2018lni       & 04:09:37.65\,$+$73:53:41.6  & 2018-12-08  &    0.138  & $-19.4$ & H+He\,(Bowen)     &  $9.94_{0.15}^{0.10}$ & 14\\
% ZTF19aabbnzo         & AT\,2018lna       & 07:03:18.64\,$+$23:01:44.6  & 2019-01-25  &    0.091  & $-19.5$ & H+He              &  $9.47_{0.09}^{0.12}$ & 14\\
% ZTF19aakswrb         & AT\,2019bhf       & 15:09:15.97\,$+$16:14:22.5  & 2019-02-25  &   0.1206  & $-20.1$ & H                 &  $10.21_{0.12}^{0.15}$ & 14\\
% ASASSN-19bt          & AT\,2019ahk       & 07:00:11.39\,$-$66:02:24.7  & 2019-03-06  &   0.0262  & $-20.7$ & H                 &  $9.74_{0.10}^{0.09}$ & 17\\
% ZTF19aakiwze         & AT\,2019cho       & 12:55:09.20\,$+$49:31:09.9  & 2019-02-21  &    0.193  & $-20.7$ & H+He\,(Bowen)     &  $10.10_{0.16}^{0.17}$ & 14\\
%  ASASSN-19dj         & AT\,2019azh       & 08:13:16.95\,$+$22:38:53.8  & 2019-03-16  &   0.0222  & $-19.9$ & H+He              &  $9.86_{0.14}^{0.15}$ & 18\\
% ZTF19aapreis         & AT\,2019dsg       & 20:57:02.97\,$+$14:12:16.2  & 2019-04-27  &   0.0512  & $-19.2$ & H+He\,(Bowen)     &  $10.36_{0.12}^{0.17}$ & 14\\
%  Gaia19bpt           & AT\,2019ehz       & 14:09:41.90\,$+$55:29:27.7  & 2019-05-08  &    0.074  & $-19.6$ & H                 &  $9.67_{0.15}^{0.09}$ & 14\\
% ZTF19abidbya         & AT\,2019lwu       & 23:11:12.30\,$-$01:00:10.8  & 2019-07-26  &    0.117  & $-19.8$ & H                 &  $9.87_{0.15}^{0.12}$ & 14\\
% ZTF19abhhjcc         & AT\,2019meg       & 18:45:16.19\,$+$44:26:18.9  & 2019-08-01  &    0.152  & $-20.2$ & H                 &  $9.69_{0.05}^{0.05}$ & 14\\
%  ATLAS19qqu          & AT\,2019mha       & 16:16:27.78\,$+$56:25:56.3  & 2019-08-09  &    0.148  & $-19.9$ & H                 &  $10.05_{0.15}^{0.11}$ & 14\\
% ZTF19abzrhgq         & AT\,2019qiz       & 04:46:37.88\,$-$10:13:34.8  & 2019-10-05  &   0.0151  & $-18.6$ & H+He\,(Bowen)     &  $10.03_{0.14}^{0.10}$ & 14\\


==> Overleaf arXiv Submission Generated source/tables/lcfit_ISSI.tex <==
SDSS-TDE2            &                 &  $44.54_{0.06}^{0.08}$ &  $4.35_{0.03}^{0.03}$ &  $0.39_{0.25}^{0.22}$ &  $54267.0             $ & --            &  $2.08_{0.08}^{0.09}$ &  $-0.7_{0.2}^{0.2}$ &  $1.51_{0.32}^{0.35}$ &  $2.32_{0.13}^{0.12}$\\
PTF-09ge             &                 &  $44.04_{0.01}^{0.01}$ &  $4.31_{0.00}^{0.00}$ &  --  &  $54992.9_{1.0}^{1.0}$ &  $1.3_{0.02}^{0.02}$ &  $1.78_{0.02}^{0.02}$ &  $-1.7_{0.2}^{0.2}$ &  $1.85_{0.10}^{0.08}$ &  $1.74_{0.03}^{0.04}$\\
PTF-09axc            &                 &  $43.46_{0.02}^{0.03}$ &  $4.08_{0.00}^{0.00}$ &  --  &  $55016.4_{6.0}^{9.3}$ &  $0.9_{0.37}^{0.23}$ &  $2.45_{0.43}^{0.39}$ &  $-1.5_{0.3}^{0.3}$ &  $2.21_{0.17}^{0.14}$ &  $2.22_{0.07}^{0.08}$\\
PTF-09djl            &                 &  $44.42_{0.04}^{0.04}$ &  $4.41_{0.00}^{0.00}$ &  --  &  $55048.3_{4.6}^{5.6}$ &  $1.1_{0.14}^{0.07}$ &  $2.12_{0.33}^{0.52}$ &  $-1.7_{0.3}^{0.2}$ &  $1.67_{0.14}^{0.11}$ &  $1.63_{0.05}^{0.06}$\\
PS1-10jh             &                 &  $44.47_{0.07}^{0.07}$ &  $4.49_{0.03}^{0.03}$ &  $0.43_{0.29}^{0.43}$ &  $55393.8_{1.4}^{1.4}$ &  $1.3_{0.02}^{0.02}$ &  $1.56_{0.03}^{0.03}$ &  $-1.5_{0.6}^{0.2}$ &  $1.44_{0.22}^{0.41}$ &  $1.55_{0.07}^{0.07}$\\
PS1-11af             &                 &  $44.16_{0.03}^{0.03}$ &  $4.31_{0.01}^{0.01}$ &  $-0.80_{0.28}^{0.39}$ &  $55578.9_{1.2}^{1.2}$ &  $0.9_{0.04}^{0.04}$ &  $1.69_{0.02}^{0.02}$ &  $-2.1_{0.5}^{0.5}$ &  $1.73_{0.17}^{0.16}$ &  $1.54_{0.09}^{0.11}$\\
ASASSN-14ae          &                 &  $43.87_{0.01}^{0.01}$ &  $4.27_{0.01}^{0.01}$ &  $0.24_{0.13}^{0.14}$ &  $56684.9             $ & --            &  $1.45_{0.01}^{0.01}$ &  $-2.4_{0.2}^{0.2}$ &  $1.52_{0.07}^{0.05}$ &  $1.21_{0.02}^{0.03}$\\
ASASSN-14li          &                 &  $43.66_{0.02}^{0.02}$ &  $4.51_{0.01}^{0.01}$ &  $-0.21_{0.07}^{0.07}$ &  $56989.4             $ & --            &  $1.77_{0.01}^{0.01}$ &  $-1.4_{0.1}^{0.1}$ &  $1.69_{0.09}^{0.09}$ &  $1.80_{0.04}^{0.04}$\\
iPTF-15af            &                 &  $44.10_{0.08}^{0.10}$ &  $4.70_{0.03}^{0.04}$ &  $1.42_{0.80}^{0.43}$ &  $57061.6_{1.8}^{1.6}$ &  $1.5_{0.03}^{0.02}$ &  $1.91_{0.02}^{0.03}$ &  $-1.6_{0.6}^{0.6}$ &  $1.91_{0.22}^{0.22}$ &  $1.91_{0.16}^{0.15}$\\
ASASSN-15oi          &                 &  $44.45_{0.01}^{0.01}$ &  $4.14_{0.01}^{0.01}$ &  $1.95_{0.09}^{0.04}$ &  $57247.9             $ & --            &  $1.39_{0.01}^{0.01}$ &  $-2.2_{0.2}^{0.2}$ &  $1.46_{0.09}^{0.07}$ &  $1.34_{0.06}^{0.06}$\\
OGLE16aaa            &                 &  $44.22_{0.01}^{0.01}$ &  $4.23_{0.00}^{0.00}$ &  $-0.11_{0.06}^{0.07}$ &  $57414.3_{1.7}^{1.5}$ &  $1.3_{0.03}^{0.03}$ &  $2.01_{0.05}^{0.06}$ &  $-2.2_{0.4}^{0.3}$ &  $2.19_{0.09}^{0.09}$ &  $2.03_{0.03}^{0.03}$\\
iPTF-16axa           &                 &  $43.82_{0.02}^{0.03}$ &  $4.37_{0.01}^{0.01}$ &  $-0.52_{0.24}^{0.29}$ &  $57523.4             $ & --            &  $1.73_{0.01}^{0.01}$ &  $-1.6_{0.2}^{0.3}$ &  $1.54_{0.16}^{0.13}$ &  $1.56_{0.06}^{0.08}$\\
iPTF-16fnl           &                 &  $43.18_{0.02}^{0.03}$ &  $4.40_{0.01}^{0.01}$ &  $-0.14_{0.13}^{0.16}$ &  $57626.5_{11.6}^{3.6}$ &  $1.3_{0.18}^{0.12}$ &  $1.36_{0.01}^{0.01}$ &  $-2.1_{0.2}^{0.2}$ &  $1.35_{0.09}^{0.08}$ &  $1.18_{0.05}^{0.05}$\\
PS17dhz              & AT\,2017eqx     &  $43.82_{0.05}^{0.03}$ &  $4.31_{0.01}^{0.01}$ &  $-0.39_{0.23}^{0.25}$ &  $57910.4_{7.1}^{3.9}$ &  $1.2_{0.20}^{0.19}$ &  $1.59_{0.02}^{0.02}$ &  $-2.0_{0.3}^{0.3}$ &  $1.47_{0.13}^{0.10}$ &  $1.31_{0.06}^{0.09}$\\
PS18kh               & AT\,2018zr      &  $43.78_{0.02}^{0.02}$ &  $4.14_{0.01}^{0.01}$ &  $0.46_{0.05}^{0.05}$ &  $58180.7_{1.0}^{1.1}$ &  $1.0_{0.03}^{0.04}$ &  $1.88_{0.03}^{0.03}$ &  $-0.8_{0.1}^{0.0}$ &  $1.23_{0.12}^{0.15}$ &  $2.14_{0.03}^{0.03}$\\
ZTF18aahqkbt         & AT\,2018bsi     &  $43.87_{0.08}^{0.08}$ &  $4.37_{0.03}^{0.03}$ &  $0.21_{0.30}^{0.63}$ &  $58217.2             $ & --            &  $1.94_{0.10}^{0.12}$ &  $-1.9_{0.6}^{0.4}$ &  $1.92_{0.21}^{0.25}$ &  $1.83_{0.07}^{0.09}$\\
ASASSN-18ul          & AT\,2018fyk     &  $44.48_{0.03}^{0.04}$ &  $4.56_{0.02}^{0.02}$ &  $-0.02_{0.12}^{0.12}$ &  $58317.5             $ & --            &  $1.99_{0.02}^{0.02}$ &  $-1.9_{0.1}^{0.1}$ &  $2.14_{0.06}^{0.06}$ &  $1.76_{0.02}^{0.03}$\\
ASASSN-18pg          & AT\,2018dyb     &  $44.16_{0.01}^{0.01}$ &  $4.37_{0.01}^{0.01}$ &  $-0.25_{0.03}^{0.03}$ &  $58346.7_{1.3}^{1.4}$ &  $1.5_{0.03}^{0.01}$ &  $1.59_{0.01}^{0.01}$ &  $-1.9_{0.1}^{0.1}$ &  $1.49_{0.05}^{0.05}$ &  $1.29_{0.03}^{0.03}$\\
ATLAS18way           & AT\,2018hco     &  $44.25_{0.04}^{0.04}$ &  $4.39_{0.01}^{0.01}$ &  $0.05_{0.09}^{0.10}$ &  $58401.8_{1.9}^{1.7}$ &  $0.9_{0.04}^{0.04}$ &  $2.03_{0.04}^{0.04}$ &  $-1.2_{0.2}^{0.2}$ &  $1.73_{0.15}^{0.16}$ &  $2.00_{0.07}^{0.06}$\\
ASASSN-18zj          & AT\,2018hyz     &  $44.11_{0.01}^{0.01}$ &  $4.25_{0.01}^{0.01}$ &  $0.18_{0.05}^{0.05}$ &  $58428.0             $ & --            &  $1.72_{0.01}^{0.01}$ &  $-1.1_{0.1}^{0.1}$ &  $1.29_{0.06}^{0.07}$ &  $1.71_{0.01}^{0.01}$\\
ATLAS18yzs           & AT\,2018iih     &  $44.62_{0.03}^{0.04}$ &  $4.23_{0.01}^{0.01}$ &  $0.19_{0.05}^{0.05}$ &  $58442.2_{0.8}^{1.6}$ &  $1.2_{0.01}^{0.01}$ &  $2.05_{0.04}^{0.04}$ &  $-0.9_{0.1}^{0.1}$ &  $1.61_{0.07}^{0.11}$ &  $2.06_{0.05}^{0.06}$\\
ZTF18actaqdw         & AT\,2018lni     &  $44.21_{0.17}^{0.29}$ &  $4.44_{0.07}^{0.09}$ &  $0.48_{0.47}^{0.46}$ &  $58460.3_{5.8}^{3.6}$ &  $0.8_{0.50}^{0.18}$ &  $2.16_{0.12}^{0.16}$ &  $-1.4_{1.6}^{0.8}$ &  $2.46_{0.45}^{0.37}$ &  $2.23_{0.19}^{0.22}$\\
ZTF19aabbnzo         & AT\,2018lna     &  $44.56_{0.06}^{0.06}$ &  $4.60_{0.02}^{0.03}$ &  $0.93_{0.92}^{0.72}$ &  $58508.3_{2.0}^{2.2}$ &  $1.2_{0.07}^{0.06}$ &  $1.65_{0.03}^{0.03}$ &  $-2.1_{0.7}^{0.7}$ &  $1.79_{0.21}^{0.24}$ &  $1.66_{0.15}^{0.16}$\\
ZTF19aakswrb         & AT\,2019bhf     &  $43.91_{0.05}^{0.04}$ &  $4.20_{0.02}^{0.02}$ &  $0.74_{0.14}^{0.15}$ &  $58539.3_{5.7}^{4.4}$ &  $0.6_{0.35}^{0.23}$ &  $1.70_{0.03}^{0.04}$ &  $-1.3_{0.4}^{0.4}$ &  $1.70_{0.20}^{0.23}$ &  $1.96_{0.09}^{0.07}$\\
ASASSN-19bt          & AT\,2019ahk     &  $44.08_{0.01}^{0.01}$ &  $4.21_{0.01}^{0.01}$ &  $0.10_{0.03}^{0.03}$ &  $58548.3_{0.9}^{0.8}$ &  $1.3_{0.01}^{0.01}$ &  $1.67_{0.01}^{0.01}$ &  $-1.6_{0.1}^{0.1}$ &  $1.66_{0.05}^{0.05}$ &  $1.72_{0.01}^{0.01}$\\
ZTF19aakiwze         & AT\,2019cho     &  $43.98_{0.01}^{0.01}$ &  $4.19_{0.01}^{0.01}$ &  $0.84_{0.23}^{0.21}$ &  $58535.3_{1.6}^{3.0}$ &  $0.8_{0.11}^{0.10}$ &  $1.94_{0.03}^{0.03}$ &  $-1.0_{0.5}^{0.4}$ &  $1.83_{0.13}^{0.25}$ &  $2.19_{0.16}^{0.13}$\\
ASASSN-19dj          & AT\,2019azh     &  $44.50_{0.02}^{0.02}$ &  $4.53_{0.01}^{0.01}$ &  $0.98_{0.19}^{0.21}$ &  $58558.6_{1.6}^{1.5}$ &  $1.3_{0.04}^{0.05}$ &  $1.83_{0.01}^{0.01}$ &  $-1.8_{0.1}^{0.2}$ &  $1.87_{0.08}^{0.08}$ &  $1.96_{0.04}^{0.05}$\\
ZTF19aapreis         & AT\,2019dsg     &  $44.26_{0.05}^{0.04}$ &  $4.49_{0.01}^{0.01}$ &  $-0.07_{0.12}^{0.14}$ &  $58600.2_{10.0}^{8.2}$ &  $1.2_{0.12}^{0.06}$ &  $1.80_{0.02}^{0.02}$ &  $-1.5_{0.1}^{0.1}$ &  $1.51_{0.10}^{0.11}$ &  $1.59_{0.06}^{0.06}$\\
Gaia19bpt            & AT\,2019ehz     &  $44.03_{0.02}^{0.01}$ &  $4.33_{0.01}^{0.01}$ &  $-0.40_{0.03}^{0.03}$ &  $58611.4_{0.6}^{0.6}$ &  $0.9_{0.02}^{0.03}$ &  $1.67_{0.01}^{0.01}$ &  $-1.8_{0.1}^{0.1}$ &  $1.73_{0.09}^{0.06}$ &  $1.61_{0.04}^{0.04}$\\
ZTF19abidbya         & AT\,2019lwu     &  $43.60_{0.04}^{0.03}$ &  $4.09_{0.01}^{0.01}$ &  $0.64_{0.19}^{0.14}$ &  $58690.2_{0.7}^{1.0}$ &  $0.4_{0.21}^{0.17}$ &  $1.68_{0.05}^{0.06}$ &  $-1.5_{0.5}^{0.4}$ &  $1.56_{0.18}^{0.20}$ &  $1.67_{0.08}^{0.09}$\\
ZTF19abhhjcc         & AT\,2019meg     &  $44.36_{0.04}^{0.03}$ &  $4.44_{0.01}^{0.01}$ &  $1.94_{0.09}^{0.05}$ &  $58696.4_{0.6}^{0.6}$ &  $0.9_{0.03}^{0.02}$ &  $1.72_{0.02}^{0.03}$ &  $-0.2_{0.5}^{0.1}$ &  $2.37_{0.66}^{0.44}$ &  $2.56_{0.18}^{0.15}$\\
ATLAS19qqu           & AT\,2019mha     &  $44.05_{0.05}^{0.06}$ &  $4.32_{0.03}^{0.03}$ &  $0.36_{1.07}^{0.88}$ &  $58704.0_{0.8}^{0.7}$ &  $1.1_{0.02}^{0.02}$ &  $1.23_{0.02}^{0.03}$ &  $-4.0_{0.5}^{0.7}$ &  $1.63_{0.12}^{0.11}$ &  $1.21_{0.09}^{0.10}$\\
ZTF19abzrhgq         & AT\,2019qiz     &  $43.44_{0.01}^{0.01}$ &  $4.28_{0.01}^{0.01}$ &  $-0.17_{0.09}^{0.10}$ &  $58761.4_{0.4}^{0.4}$ &  $0.8_{0.01}^{0.01}$ &  $1.48_{0.01}^{0.01}$ &  $-2.0_{0.1}^{0.1}$ &  $1.40_{0.06}^{0.06}$ &  $1.26_{0.03}^{0.02}$\\

